When to Prune? A Policy towards Early Structural Pruning

Pruning enables appealing reductions in network memory footprint and time complexity. Conventional post-training pruning techniques lean towards efficient inference while overlooking the heavy computation for training. Recent exploration of pre-training pruning at initialization hints on training cost reduction via pruning, but suffers noticeable performance degradation. We attempt to combine the benefits of both directions and propose a policy that prunes as early as possible during training without hurting performance. Instead of pruning at initialization, our method exploits initial dense training for few epochs to quickly guide the architecture, while constantly evaluating dominant sub-networks via neuron importance ranking. This unveils dominant sub-networks whose structures turn stable, allowing conventional pruning to be pushed earlier into the training. To do this early, we further introduce an Early Pruning Indicator (EPI) that relies on sub-network architectural similarity and quickly triggers pruning when the sub-network's architecture stabilizes. Through extensive experiments on ImageNet, we show that EPI empowers a quick tracking of early training epochs suitable for pruning, offering same efficacy as an otherwise ``oracle'' grid-search that scans through epochs and requires orders of magnitude more compute. Our method yields $1.4\%$ top-1 accuracy boost over state-of-the-art pruning counterparts, cuts down training cost on GPU by $2.4\times$, hence offers a new efficiency-accuracy boundary for network pruning during training.

==> speedup_fig.tex <==
\begin{figure}[!t]
% \resizebox{\linewidth}{!}{
\centering

\resizebox{0.85\columnwidth}{!}{
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{c}
% \includegraphics[width=1.3\linewidth]{latex/figures/policy-legend.png}\\
% \includegraphics[width=1.3\linewidth]{latex/figures/resnet50-theoretical-speedup.png}\\
% (a) Theoretical Training Speed Up on ResNet50\vspace{4mm}\\
\includegraphics[width=\columnwidth]{figures/resnet50-actual-speedup}\\
\end{tabular}
}    
\caption{Actual training speed-ups on ResNet50 with different prune ratios using different pruning policies. Actual speed measured on an NVIDIA TITAN V GPU at batch size $64$. Top-right corner is preferred.}  \vspace{-5mm}
    \label{fig:policy-compare}
\end{figure}




% \begin{figure}[!t]
% % \resizebox{\linewidth}{!}{
% \centering

% \resizebox{.84\linewidth}{!}{
% \begingroup
% \renewcommand*{\arraystretch}{0.3}
% % \setlength\extrarowheight{-30pt}
% \begin{tabular}{c}
% \vspace{-5mm}
% \includegraphics[width=1.3\linewidth]{latex/figures/policy-legend.png}\\
% \includegraphics[width=1.3\linewidth]{latex/figures/resnet50-theoretical-speedup.png}\\
% (a) Theoretical Training Speed Up on ResNet50\vspace{4mm}\\
% \includegraphics[width=1.3\linewidth]{latex/figures/resnet50-actual-speedup.png}\\
% (b) Actual Training Speed Up on ResNet50 \\
% \vspace{-2mm}
% \end{tabular}
% \endgroup
% }    
% \caption{Theoretical and actual training speed-ups on ResNet50 with different prune ratios using different pruning policies. Actual speed measured on an NVIDIA TITAN V GPU at batch size $64$. Top right corner is preferred.} \vspace{-5mm}
%     \label{fig:policy-compare}
% \end{figure}

%         \includegraphics[width=0.8\linewidth]{latex/figures/policy-legend.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{.5\textwidth}
%         \centering
%          \includegraphics[width=0.8\linewidth]{latex/figures/resnet50-theoretical-speedup.png}
%          \caption{\small{Theoretical Training Speed Up on ResNet50}}
%          \label{fig:theoretical-speedup}
%     \end{subfigure}
%     \begin{subfigure}[b]{.5\textwidth}
%         \centering
%          \includegraphics[width=0.8\linewidth]{latex/figures/resnet50-actual-speedup.png}
%          \caption{\small{Actual Training Speed Up on ResNet50}}
%          \label{fig:actual-speedup}
%     \end{subfigure}
%     % }
%     \caption{Theoretical and actual training speed-ups on ResNet50 with different prune ratios using different pruning policies. Actual speed measured on an NVIDIA TITAN V GPU at batch size $64$. Top right corner is preferred.} 
%     \label{fig:policy-compare}
% \end{figure}




% \begin{figure}[!t]
% % \resizebox{\linewidth}{!}{
% \centering
%     % \begin{subfigure}[b]{0.8\textwidth}
%     % \includegraphics[width=0.8\linewidth]{latex/figures/policy-legend.png}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{latex/figures/policy-legend.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{.5\textwidth}
%         \centering
%          \includegraphics[width=0.8\linewidth]{latex/figures/resnet50-theoretical-speedup.png}
%          \caption{\small{Theoretical Training Speed Up on ResNet50}}
%          \label{fig:theoretical-speedup}
%     \end{subfigure}
%     \begin{subfigure}[b]{.5\textwidth}
%         \centering
%          \includegraphics[width=0.8\linewidth]{latex/figures/resnet50-actual-speedup.png}
%          \caption{\small{Actual Training Speed Up on ResNet50}}
%          \label{fig:actual-speedup}
%     \end{subfigure}
%     % }
%     \caption{Theoretical and actual training speed-ups on ResNet50 with different prune ratios using different pruning policies. Actual speed measured on an NVIDIA TITAN V GPU at batch size $64$. Top right corner is preferred.} 
%     \label{fig:policy-compare}
% \end{figure}

==> tables/table1.tex <==
\label{sec:epi-guided-pruning-result}
\begin{table}[!t]
    \centering
    \begin{minipage}{\columnwidth}
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \multicolumn{1}{c}{}& \multirow{2}{*}{\textbf{Network(s)}} & \multicolumn{4}{c}{\textbf{Starting epoch for pruning}} \\  \cline{3-6}
        
        % \multicolumn{1}{c}{}& & \multirow{2}{*}{EPI (ours)}  & \multirow{2}{*}{random} & \multicolumn{2}{c}{heuristic}\\
        \multicolumn{1}{c}{}&  & Random & Init.~\cite{de2020force, lee2018snip} & Pre-defined~\cite{Frankle2020earlyphase}  &  EPI (ours) \\
        \midrule
        \multirow{4}{*}{\begin{sideways}\textbf{\footnotesize{Magnitude}}\end{sideways}  } & ResNet50 & $0.940$ & $3.604$ & $0.115$ & $\mathbf{0.091}$ \\
        & ResNet34 & $0.267$ & $0.838$ & $0.353$ & $\mathbf{0.169}$ \\
        & MobileNet-v1 & $6.285$ & -- & $0.135$ & $\mathbf{0.135}$ \\    
        \cline{2-6}
        & Overall & $2.497$ & $2.221$ & $0.201$ & $\mathbf{0.132}$ \\
        \midrule
        \multirow{4}{*}{\begin{sideways}\textbf{\footnotesize{Gradient}}\end{sideways}  } & ResNet50 & $0.992$  & $2.738$ & $0.267$ & $\mathbf{0.092}$ \\
        & ResNet34 & $0.153$ & $\mathbf{0.122}$ & $0.221$ & $0.195$ \\
        & MobileNet-v1 & $0.132$ & $0.186$ & $\mathbf{0.110}$ & $0.178$ \\
        \cline{2-6}
        & Overall & $0.426$ & $1.015$ & $0.199$ & $\mathbf{0.155}$ \\
        \bottomrule
    \end{tabular}
    }
    \end{minipage}
    \caption{Absolute top-1 accuracy change relative to the results per oracle grid search for optimal pruning starting point. %Average Top1 accuracy drop (in \%) of our method and the baselines for magnitude and gradient-based pruning on ImageNet. 
    Lower is better. Init. refers to pruning at initialization using a structural version of FORCE~\cite{de2020force}, also equivalent to the structural and iterative SNIP~\cite{lee2018snip}. Pre-define refers to heuristically pre-define a pruning start epoch $30$, which we found empirically the last epoch not leading to a significant accuracy drop. This is aligned with~\cite{frankle2019linear} where the authors propose to wait for several training iterations before pruning.}
     \vspace{-0.3cm}
    \label{tab:policy-compare}
\end{table}
%, we heuristically pre-define a pruning start epoch $30$, which we found empirically the last epoch not leading to a significant accuracy drop.

% \label{sec:epi-guided-pruning-result}
% \begin{table}[!t]
%     \centering
%     \begin{minipage}{\columnwidth}
%     \resizebox{.99\columnwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \cline{2-6}
%         \multicolumn{1}{c|}{}& \multirow{3}{*}{network(s)} & \multicolumn{4}{c|}{acc drop (\%) compared to grid search $\downarrow$} \\  \cline{3-6}
%         \multicolumn{1}{c|}{}& & \multirow{2}{*}{Ours}  & \multirow{2}{*}{random} & \multicolumn{2}{c|}{heuristic}\\
%         \multicolumn{1}{c|}{}&  &   &  & at 0\footnote{\label{note1}Pruning at 0 is a structured version of FORCE~\cite{de2020force}, also equivalent to structured and iterative SNIP~\cite{lee2018snip}} & at 30  \\
%         \hline
%         \multirow{4}{*}{\begin{sideways}magnitude\end{sideways}  } & resnet50 & 0.091 & 0.940 & $3.604$\footnote{\label{note2}{refers to pruning with a larger pruning ratio that made the network not-trainable. ``--'' means all prunings lead to not-trainable network.}} & 0.115\\
%         & resnet34 & 0.169 & 0.267 & 0.838\footref{note2} & 0.353\\
%         & mobilenet-v1 & 0.135 & 6.285 & --\footref{note2} & 0.135\\    
%         \cline{2-6}
%         & average\footnote{\label{note3}refers to the accuracy drop averaged over the three networks.} & \textbf{0.132} & 2.497 & 2.221 & 0.201 \\
%         \hline\hline
%         \multirow{4}{*}{\begin{sideways}gradient\end{sideways}  } & resnet50 & 0.092 & 0.992  & 2.738 & 0.267\\
%         & resnet34 & 0.195 & 0.153 & 0.122 & 0.221\\
%         & mobilenet-v1 & 0.178 & 0.132 & 0.186 & 0.110\\
%         \cline{2-6}
%         & average\footref{note3} & \textbf{0.155} & 0.426 & 1.015 & 0.199\\
%         \hline
%     \end{tabular}
%     }
%     \end{minipage}
%     \caption{Policy comparison. Average Top1 accuracy drop (in \%) of our method and the baselines for magnitude and gradient-based pruning on ImageNet. Lower is better.}
%     \label{tab:policy-compare}
% \end{table}

==> tables/table2.tex <==
\begin{table}[!t]
    \centering
    %\begin{minipage}{\columnwidth}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{cccccc}
        % \cline{2-6}
        \toprule
        % \multicolumn{1}{c}{} & \multirow{2}{*}{\textbf{Method}} & $50\%$ \textbf{Pruned} & 
        % \multirow{2}{*}{\textbf{FLOPs (G)}} & \multirow{2}{*}{$\%$ \textbf{FLOPs} $\downarrow$} & \textbf{Pruning}\\
        % \multicolumn{1}{c}{} &  & \textbf{Top1 Acc.} & & & \textit{at epoch}\\
        % \hline
        
        & \textbf{Method} & \textbf{Top-1 acc.} $\uparrow$ & \textbf{FLOPs (G)}$\downarrow$ & \textbf{FLOPs reduc.(\%)} $\uparrow$ & \textbf{Starting epoch} $\downarrow$ \\
        \midrule
        
        \multirow{2}{*}{\textbf{ResNet34}} & GPWP~\cite{GPWP} & $\mathbf{73.64}$ & $3.087$ & $15.90$ & $40$\\
        % & FORCE~\cite{de2020force} & 73.58 & 3.144 & 14.20 & 0 \\
        & PaT \textbf{(ours)} & $73.50$ & $\mathbf{2.911}$ & $\mathbf{20.70}$ & $\mathbf{11}$ \\
        % & ours & 74.36 & 72.44 & 1.92 & \textbf{2.283} & \textbf{37.81} \\ 
        \midrule
        \multirow{3}{*}{\textbf{ResNet50}} & PT~\cite{lym2019prunetrain} & $74.73$ & $2.303$ & $44.00$ & $90$ \\
        & LFPC~\cite{he2020learning} & $74.18$  & $\mathbf{1.612}$ & $\mathbf{60.80}$ & $35$\\
        % & FORCE~\cite{de2020force} & 73.73 & 2.359 & 42.16 & 0 \\
        & PaT \textbf{(ours)} & $\mathbf{74.85}$ & $1.695$ & $58.78$ & \textbf{13}\\
        \hline
        
    \end{tabular}
    }
    %\end{minipage}
    \footnotesize
    \caption{Comparison with state-of-the-art in-training pruning methods. For a fair comparison we report here $10\%$ filter pruning for ResNet34 and $40\%$ filter pruning for ResNet50 as literature.
    }
    \vspace{-0.5cm}
    \label{tab:prune-during-training-compare}
\end{table}



% \begin{table}[!t]
%     \centering
%     %\begin{minipage}{\columnwidth}
%     \resizebox{\columnwidth}{!}{
%         \begin{tabular}{|c|c|c|c|c|c|}
%         \cline{2-6}
%         \multicolumn{1}{c|}{} & \multirow{2}{*}{Method} & \% Pruned & 
%         \multirow{2}{*}{FLOPs (G)} & \multirow{2}{*}{\% FLOPs $\downarrow$} & Prune ends\\
%         \multicolumn{1}{c|}{} &  & Top1 Acc. & & & at epoch\\
%         \hline
%         \multirow{2}{*}{\begin{sideways}RN34\end{sideways}} & GPWP~\cite{GPWP} & \textbf{73.64} & 3.087 & 15.90 & 40\\
%         & ours & 73.50 & \textbf{2.911} & \textbf{20.70} & \textbf{11} \\
%         % & ours & 74.36 & 72.44 & 1.92 & \textbf{2.283} & \textbf{37.81} \\ 
%         \hline
%         \hline
%         \multirow{3}{*}{\begin{sideways}RN50\end{sideways}} & PruneTrain~\cite{lym2019prunetrain} & 74.73 & 2.303 & 44.00 & 90 \\
%         & LFPC~\cite{he2020learning} & 74.18  & \textbf{1.612} & \textbf{60.80} & 35\\
%         & ours & \textbf{74.85} & 1.695 & 58.78 & \textbf{13}\\
%         \hline
        
%     \end{tabular}
%     }
%     %\end{minipage}
%     \footnotesize
%     \caption{Comparison of pruning during training methods. 
%     }
%     \label{tab:prune-during-training-compare}
% \end{table}

